Harder, Better, Faster, Stronger: The $\Delta(1232)$ Resonance in Supernova QCD Axion Emission

The high-energy tail of supernova axion emission controls searches whose response grows with axion energy. We identify a novel production channel, in which the axion is emitted through an intermediate $\Delta(1232)$ resonance, which adds a hard component to the spectrum. We calculate the axion production rate from nucleon-nucleon Bremsstrahlung in chiral effective field theory through next-to-leading order. Including the $\Delta(1232)$ roughly doubles the luminosity at one second after bounce and increases the number of escaping axions above $200$ MeV by a factor of about $3$ over the first nine seconds, relative to the nucleon-only calculation. Adding this new production channel roughly doubles $\gamma$-ray counts from conversion in the progenitor's magnetic field and increases water-Cherenkov counts by about an order of magnitude through its combined effects on emission and absorption. The same hard component can mimic a higher core temperature or thermal-pion emission in $\gamma$-ray spectral fits. The $\Delta(1232)$ resonance is therefore crucial for predicting supernova axion signals and interpreting their spectra.

==> latexmkrc <==
# The Letter (main.tex) and the SM (supplement.tex) read each other's labels with xr-hyper. Overleaf names the
# output of the compiled document output.aux, so the other document's .aux is written here with one fast pdflatex
# pass in draft mode (no PDF, no figures, no bibliography) whenever its .tex has changed.
add_cus_dep('tex', 'aux', 0, 'makeexternaldocument');
sub makeexternaldocument {
    my $doc = $_[0];
    if (($doc eq 'main' || $doc eq 'supplement') && $root_filename ne $doc) {
        system("pdflatex -draftmode -interaction=batchmode \"$doc.tex\"");
    }
    return 0;
}

